SurFree: a fast surrogate-free black-box attack

Machine learning classifiers are critically prone to evasion attacks. Adversarial examples are slightly modified inputs that are then misclassified, while remaining perceptively close to their originals. Last couple of years have witnessed a striking decrease in the amount of queries a black box attack submits to the target classifier, in order to forge adversarials. This particularly concerns the black-box score-based setup, where the attacker has access to top predicted probabilites: the amount of queries went from to millions of to less than a thousand. This paper presents SurFree, a geometrical approach that achieves a similar drastic reduction in the amount of queries in the hardest setup: black box decision-based attacks (only the top-1 label is available). We first highlight that the most recent attacks in that setup, HSJA, QEBA and GeoDA all perform costly gradient surrogate estimations. SurFree proposes to bypass these, by instead focusing on careful trials along diverse directions, guided by precise indications of geometrical properties of the classifier decision boundaries. We motivate this geometric approach before performing a head-to-head comparison with previous attacks with the amount of queries as a first class citizen. We exhibit a faster distortion decay under low query amounts (few hundreds to a thousand), while remaining competitive at higher query budgets.

==> 6_Notes.tex <==
% !TEX root =  fastbbearl.tex
\pagebreak
\pagebreak
\section{Notes}
Some notes (to be removed before submitting).

Papers to be cited: \cite{Chen:2017aa}, \cite{Ilyas:2018aa}, \cite{Tu:2019aa}, \cite{Narodytska:2017aa},
\cite{Guo:2019aa}, \cite{Cheng:2019aa}, \cite{Zhao:2020aa}, \cite{Chen:2020aa}, \cite{Rahmati:2020aa},
\cite{Li:2020aa}, \cite{Brendel:2018aa}

By historical order:
\medskip

{\color{red}
\textbf{Summary of \cite{Narodytska:2017aa}:}
\begin{itemize}
\item Very old. Output $ = P(y|x)$.
\item Gradient free estimation
\item 70 sec. to forge 1 image on ImageNet. Distortion $L_1$.
\end{itemize}}

\medskip

{\color{red}
\textbf{Summary of ZOO, \cite{Chen:2017aa}:}
\begin{itemize}
\item Gives some arguments about 'substitute model approaches'
\item use a coordinate descend based method.
\item use dimension reduction (DCT or bilinear upscaling)
\item use hierarchical dimension reduction (from small to larger dimension) for targeted attack.
\item Output $= P(y|x)$
\item approximate gradient 
\item use `importance' sampling (sample pixel in the center because they matter more than in the corner).
\item $1,500$ iterations means $1,500\times 128$ gradients estimations, $1,500\times 128 \times 3$ calls. 20 minutes per image!
\item Average $L_2$ is 3 times larger than C\&W (white-box). 
\item targeted and untargeted
\end{itemize}}

\medskip

\textbf{Summary of BA~\cite{Brendel:2018aa}}:
\begin{itemize}
\item First fully `decision-based' paper (or hard label).
\item very close to our approach
\item distortion (median of power) is the same order of white-box attack (C\&W or DeepFool)
\item example of images from some increasing numbers of calls
\item $1,200,000$ calls! (page 7).
\item Figure 6: distortion vs. calls.
\item targeted and untargeted. Targeted $=$ initialize with image of the target class.
\end{itemize}

\medskip

\textbf{Summary of \cite{Ilyas:2018aa}:}
\begin{itemize}
\item Some references about `substitute model approaches' do not work so well.
\item Encompass `partial information setting' (ie. $P(y|x)$) and `$k$-labels only' setting (including $k=1$).
\item need a surrogate of $P(y|x)$ in the `$k$-labels only' setting
\item Estimate gradient (NES estimator) and run a PGD like white-box attack
\item With probability $1/2$, needs more than 2.7 millions of calls per image!
\item No mention about the distortion
\end{itemize}

\medskip

\textbf{Summary of OPT~\cite{Cheng:2019aa}}:
\begin{itemize}
\item truly hard label black box
\item Clever line search / dichotomy
\item ZOO - gradient estimation based on the \emph{direction}
\item 100 ImageNet, 100\% success, average $L_2$
\item $70,000$ queries ay least!
\end{itemize}

\medskip

{\color{red}
\textbf{Summary of \cite{Guo:2019aa}}:
\begin{itemize}
\item not hard label. Output $= P(y|x)$
\item around some thousands queries
\item DCT transform
\end{itemize}}

\medskip

{\color{red}
\textbf{Summary of \cite{Tu:2019aa}}:
\begin{itemize}
\item not hard label. Output $= P(y|x)$
\item ZOO with gradient estimation
\item More than $10,000$ queries.
\end{itemize}}

\medskip

{\color{red}
\textbf{Summary of \cite{Ilyas:2019aa}}:
\begin{itemize}
\item not hard label. Output $= P(y|x)$
\item gradient estimation problem
\item estimate gradient and run PGD.
\item quite efficient: less than  $1,000$ queries.
\end{itemize}}

\medskip

{\color{red}
\textbf{Summary of \cite{Zhao:2020aa}}:
\begin{itemize}
\item not hard label. Output $= P(y|x)$
\item ZOO with gradient estimation
\item quite efficient: less than  $1,000$ queries.
\end{itemize}}

\medskip

\textbf{Summary of HopSkipJump~\cite{Chen:2020aa}}:
\begin{itemize}
\item Hard label.
\item gradient estimation from hard label
\item Nice explanation with stationary point
\item Distortion for 1K, 5K, and 20K queries
\item soft plots in Fig.3 because median
\item Success rate vs. Distortion in Fig. 5 for 1K and 5K queries
\item Visualized trajectories of images 
\end{itemize}

\medskip

\textbf{Summary of GeoDA~\cite{Rahmati:2020aa}}:
\begin{itemize}
\item Hard label.
\item gradient estimation from hard label
\item comparison with HSJA and BA
\item Distortion for 1K, 5K, and 20K queries
\item soft plots in Fig.3 because mean
\item Success rate vs. Distortion in Fig. 5 for 1K and 5K queries
\item Visualized trajectories of images 
\end{itemize}

\medskip

\textbf{Summary of QEBA~\cite{Li:2020aa}}:
\begin{itemize}
\item Hard label.
\item gradient estimation from hard label
\item comparison with HSJA and BA
\item Fixed query number, target distortion, measure proba of success
\item soft plots in Fig.3 because mean
\item some ref about improvement of BA
\item Visualized trajectories of images 
\end{itemize}



\pagebreak


==> aaa <==
The literature on adversarial examples is divided into two shares, depending on the threat model: either the a\
ttacker has full knowledge of the target classifier \cite{calini2017towards} (white-box setting) or she/he has\
 an unrestricted query access to the unknown classifier \cite{Narodytska:2017aa,Brendel:2018aa,Li:2020aa,Rahma\
ti:2020aa,Chen:2020aa,Zhao:2020aa,Ilyas:2019aa,Tu:2019aa,Guo:2019aa,Cheng:2019aa,Ilyas:2018aa,Chen:2017aa} (bl\
ack-box setting).
The latter scenario is deemed as more relevant to gauge the intrinsic robustness of classifiers in real-world \
applications (typically queried through an API).

